The Modality Focusing Hypothesis: Towards Understanding Crossmodal Knowledge Distillation

Crossmodal knowledge distillation (KD) extends traditional knowledge distillation to the area of multimodal learning and demonstrates great success in various applications. To achieve knowledge transfer across modalities, a pretrained network from one modality is adopted as the teacher to provide supervision signals to a student network learning from another modality. In contrast to the empirical success reported in prior works, the working mechanism of crossmodal KD remains a mystery. In this paper, we present a thorough understanding of crossmodal KD. We begin with two case studies and demonstrate that KD is not a universal cure in crossmodal knowledge transfer. We then present the modality Venn diagram to understand modality relationships and the modality focusing hypothesis revealing the decisive factor in the efficacy of crossmodal KD. Experimental results on 6 multimodal datasets help justify our hypothesis, diagnose failure cases, and point directions to improve crossmodal knowledge transfer in the future.

==> 3-1.method.tex <==
\section{On the Efficacy of Multimodal Knowledge Distillation}\label{sec.efficacy}
\subsection{Problem Formulation}\label{sec.problem}


%The core idea of knowledge distillation is a student-teacher learning framework, where a student network is trained to mimic a teacher network. In conventional knowledge distillation, the student and teacher network receive input from the same modality (\eg, a visual student learns from a visual teacher). Multimodal knowledge distillation extends the problem by having teacher and student network take input from distinct modality combinations (\eg, an audio-visual teacher distills knowledge to a visual student).

% Formally, denote the student and teacher network by $f_S(\mathbf x_S)$ and $f_T(\mathbf x_T)$, where $\mathbf x_S$ and $\mathbf x_T$ represent student and teacher network input, respectively. Without loss of generalizability, we limit our discussion to two modalities, denoted by $x_1$ and $x_2$. The problem definition is given below.

% In this paper, we limit our consideration of KD to the supervised $K$-class classification task. Formally, the student and teacher networks are denoted by $\mathbf{f}_{\boldsymbol{\theta}_S}(\mathbf{x}_S)\in\mathbb{R}^H$ and $\mathbf{f}_{\boldsymbol{\theta}_T}(\mathbf{x}_T)\in\mathbb{R}^H$, respectively, where $\{\boldsymbol{\theta}_S,\boldsymbol{\theta}_T\}$ represent learnable parameters, and $\mathbf{x}_S\in\mathbb{R}^s$ and $\mathbf{x}_T\in\mathbb{R}^t$ are respectively inputs of the two networks. Without loss of generality, we limit our discussion within two modalities denoted by `1' (e.g., image) and `2' (e.g., audio), and the student network always takes unimodal input data from modality `1': $\mathbf{x}_S\leftarrow\mathbf{x}^1$. Consider the modality of teacher's input, there are three scenarios: (i) unimodal KD: $\mathbf{x}_T\leftarrow \mathbf{x}^1$, (ii) multimodal KD: $\mathbf{x}_T\leftarrow (\mathbf{x}^1,\mathbf{x}^2)$, and (iii) crossmodal KD: $\mathbf{x}_T\leftarrow \mathbf{x}^2$.

Below we revisit the basics of KD and introduce notations used throughout the paper.

Consider a supervised $K$-class classification problem. We denote the input of the student and teacher networks by $\mathbf{x}_S$ and $\mathbf{x}_T$, respectively. We use $\mathbf{f}_{\boldsymbol{\theta}_S}(\mathbf{x}_S)\in\mathbb{R}^K$ and $\mathbf{f}_{\boldsymbol{\theta}_T}(\mathbf{x}_T)\in\mathbb{R}^K$ to respectively represent the output (\ie, class probabilities) of the student and teacher networks, where  $\{\boldsymbol{\theta}_S,\boldsymbol{\theta}_T\}$ are learnable parameters. Without loss of generality, we limit our discussion within input data of two modalities, denoted by $\mathbf{x}_1$ and $\mathbf{x}_2$ for modality $1$ and $2$, respectively. Assume that we aim to learn a student network that takes $\mathbf{x}_1$ as input. There are three typical ways of distillation: (i) unimodal KD: the student and teacher network receive input from the same modality (\eg, a visual teacher distills knowledge to a visual student), (ii) multimodal KD: we adopt a multimodal teacher for distillation (\eg, an audio-visual teacher and a visual student), and (iii) crossmodal KD: the teacher and student network receive input from distinct modalities (\eg, an audio teacher and a visual student). 

% \textbf{Unimodal KD} Both the teacher and student take inputs from the same modality: $\mathbf{x}_S,\mathbf{x}_T\leftarrow \mathbf{x}^1$. Assume a set of paired data $D=\{(\mathbf{x}_n^1,y_n)\}_{n=1}^N$ are given, where $\mathbf{x}_n^1$ represents the $n$-th input data of modality `1', and $y_n\in\{0,1,\cdots,K-1\}$ represents the traget label. With an available teacher model, the training of student is realized by minimizing:
% \begin{equation}\label{eq.general_kd_loss}
% \begin{aligned}
%         \mathcal L &= \rho \mathcal{L}_{task} + (1-\rho) \mathcal{L}_{kd}\\
% \end{aligned}
% \end{equation}
% where $\rho\in[0,1]$ weighs the importance of two terms $\mathcal{L}_{task}$ and $\mathcal{L}_{kd}$ (i.e., driving the student to true labels or teacher's soft predictions):
% \begin{equation}
% \begin{aligned}
%     \mathcal{L}_{task} &=\sum_{n=1}^N CE(\mathbf{f}_{\boldsymbol{\theta}_S}(\mathbf{x}_n^1),y_n) \quad\text{and}\quad    \mathcal{L}_{kd} &= \sum_{n=1}^N KL(\mathbf{f}_{\boldsymbol{\theta}_S}(\mathbf{x}_n^1),\mathbf{f}_{\boldsymbol{\theta}_T}(\mathbf{x}_n^1))
% \end{aligned}
% \end{equation}

\textbf{Unimodal KD.} ($\mathbf{x}_T \leftarrow \mathbf{x}_1,\mathbf{x}_S\leftarrow \mathbf{x}_1$) Both the teacher and student take unimodal data $\mathbf{x}_1$ as input. With an available teacher model, the training of student is achieved by minimizing:
\begin{align}\label{eq.general_kd_loss}
        \mathcal L = \rho \mathcal{L}_{task} & + (1-\rho) \mathcal{L}_{kd}\\
        \mathcal{L}_{task} = \text{CE}(\mathbf{y}, \mathbf{f}_{\boldsymbol{\theta}_S}(\mathbf{x}_1)) & \quad\text{and}\quad    \mathcal{L}_{kd} =  \text{KL}(\mathbf{f}_{\boldsymbol{\theta}_T}(\mathbf{x}_1),\mathbf{f}_{\boldsymbol{\theta}_S}(\mathbf{x}_1))
\end{align}    
where $\mathbf{y}$ represents the ground truth label, $\rho\in[0,1]$ weighs the importance of two terms $\mathcal{L}_{task}$ and $\mathcal{L}_{kd}$ (\ie, driving the student to true labels or teacher's soft predictions), respectively. `CE' denotes cross entropy, and `KL' represents KL divergence.


\textbf{Multimodal KD.} ($\mathbf{x}_T\leftarrow (\mathbf{x}_1,\mathbf{x}_2), \mathbf{x}_S\leftarrow \mathbf{x}_1$) Multimodal KD resorts to a multimodal teacher in the distillation. The teacher takes multimodal data as input while the student input remains the same as in unimodal KD (\ie, $\mathbf{x}_1$). We still minimize Eq.  (\ref{eq.general_kd_loss}) to train a student model, but now $\mathcal L_{kd}$ is given by:
\begin{equation}
    \mathcal{L}_{kd} = \text{KL}(\mathbf{f}_{\boldsymbol{\theta}_T}(\mathbf{x}_1, \mathbf{x}_2),\mathbf{f}_{\boldsymbol{\theta}_S}(\mathbf{x}_1))
\end{equation}

% \textbf{Multimodal KD} In multimodal KD, a multimodal teacher network distills information to a unimodal student. The teacher model now takes multimodal data as inputs: $\mathbf{x}_T\leftarrow (\mathbf{x}^1,\mathbf{x}^2)$, while the student takes only unimodal data: $\mathbf{x}_S\leftarrow \mathbf{x}^1$. Suppose a set of paired data $D=\{(\mathbf{x}_n^1,\mathbf{x}_n^2,y_n)\}_{n=1}^N$ are given. We still minimize Eq (\ref{eq.general_kd_loss}) to train a student model, but now the second KD loss is given by:
% \begin{equation}
%     \mathcal{L}_{kd} = \sum_{n=1}^N KL(\mathbf{f}_{\boldsymbol{\theta}_S}(\mathbf{x}_n^1),\mathbf{f}_{\boldsymbol{\theta}_T}(\mathbf{x}_n^1,\mathbf{x}_n^2))
% \end{equation}

\textbf{Crossmodal KD.} ($\mathbf{x}_T\leftarrow\mathbf{x}_2$, $\mathbf{x}_S\leftarrow\mathbf{x}_1$) Crossmodal KD refers to the case where teacher and student input modalities do not overlap. It could be regarded as a special case of multimodal KD when the teacher only takes input from modality $2$. Eq. (\ref{eq.general_kd_loss}) is still valid with a slight correction to $\mathcal{L}_{kd}$: 
\begin{equation}
    \mathcal{L}_{kd} =  \text{KL}(\mathbf{f}_{\boldsymbol{\theta}_T}(\mathbf{x}_2),\mathbf{f}_{\boldsymbol{\theta}_S}(\mathbf{x}_1))
\end{equation}

% In all three cases, the training of teacher and the KD process (i.e., training of student) could be on two different datasets. Also, the target $y_n$ is not necessary for the KD process, i.e., $\rho=0$ in Eq (\ref{eq.general_kd_loss}).


% [Unimodal distillation] Both the teacher and student takes $x_2$ as input, \ie, $\mathbf x_T = \mathbf x_S = x_2$. Following \citep{}, the distillation objective measures the difference between student and teacher output, as given below:

% \begin{equation}
%     \mathcal L_{kd} = KL(f_T(x_2), f_S(x_2))
% \end{equation}

% where $KL$ represents the KL divergence, $f_T(\cdot)$ and $f_S(\cdot)$ are soft labels (\ie, class probabilities) produced by the teacher and student network. 

% [Multimodal distillation] A multimodal network is adopted as the teacher to distill information to a unimodal student, \ie, $\mathbf x_T = (x_1, x_2), \mathbf x_S = x_2$. The distillation objective takes the form of:
% \begin{equation}
%     \mathcal L_{kd} = KL(f_T(x_1, x_2), f_S(x_2))
% \end{equation}

% [Crossmodal distillation] It can be viewed as a special case of multimodal distillation, where teacher takes input from one modality and student takes input from another modality, \ie, $\mathbf x_T = x_1, \mathbf x_S = x_2$. In a more general sense, crossmodal distillation refers to the case where teacher and student input modality do not overlap. The distillation objective is provided below.

% \begin{equation}
%     \mathcal L_{kd} = KL(f_T(x_1), f_S(x_2))
% \end{equation}

% The overall loss function for training a student network is a combination of student task loss and the distillation loss, as given by:
% \begin{equation}
%     \mathcal L = \alpha \mathcal L_{task} + (1-\alpha) \mathcal L_{kd}
% \end{equation}
% where $\mathcal L_{task}$ denotes a task loss (\eg, cross entropy between student prediction and ground truth label) and $\alpha$ is a hyperparameter controlling the relative importance of two loss terms.

\subsection{Is a Multimodal Teacher Better than a Unimodal One?}\label{sec.failurecase}
Benefiting from the great representation power of multimodal data, a multimodal network usually enjoys a higher accuracy than its unimodal counterpart~\citep{mmsurvey}. This motivates many research works \citep{luo2018graph,medical1,valverde2021there} to replace conventional unimodal KD with multimodal KD, in an attempt to improve student network performance. Their underlying motivation is intuitive: {a more accurate teacher can lead to a better student. Also, the complementary modality-dependent information brought by the teacher network may further enhance student performance.} However, in this paper, we reflect on this assumption and ask the question: \emph{Is multimodal KD always more effective than unimodal KD?}

% a more accurate teacher network leads to a better student. Moreover, one might also expect that the multimodal teacher provides complementary modality-dependent information for the student to learn; this can further enhance student performance.


% With all these evidence, it seems natural to conclude that multimodal KD is superior to unimodal KD. However, does the conclusion always hold true? In spite of the great empirical success reported in prior works \citep{}, we ask one fundamental question in this paper: \emph{Is multimodal KD always effective?} Below we provide a comparison of multimodal KD with unimodal KD and describe two failure cases of multimodal KD. 
\begin{table}[!h]
\begin{center}
\caption{Evaluation of unimodal KD (UM-KD) and multimodal KD (MM-KD) on AV-MNIST and NYU Depth V2. `Mod.' is short for modality, and \texttt{A}, \texttt{I}, \texttt{RGB}, \texttt{D} represents audio, grayscale images, RGB images and depth images, respectively.}
\label{table:headings}
\begin{tabular}{cclclclcl}
\toprule
 & \multicolumn{4}{c}{AV-MNIST} & \multicolumn{4}{c}{NYU Depth V2} \\
 \cmidrule(lr){2-5}
\cmidrule(lr){6-9}
 & \multicolumn{2}{c}{Teacher} & \multicolumn{2}{c}{Student} & \multicolumn{2}{c}{Teacher} & \multicolumn{2}{c}{Student} \\
 & Mod. & Acc. (\%) & Mod. & Acc. (\%) & Mod. & mIoU (\%) & Mod. & mIoU (\%)\\
\midrule
 No-KD & - & - & \texttt{A} &68.36 & - & - & \texttt{RGB} & 46.36 \\
 UM-KD & \texttt{A} & 84.57 & \texttt{A} & 70.10 & \texttt{RGB} & 46.36 & \texttt{RGB} &48.00 \\
 MM-KD & \texttt{I} + \texttt{A} & 91.61 (\uu) & \texttt{A} & 69.73 (\dd) & \texttt{RGB} + \texttt{D} & 51.00 (\uu) & \texttt{RGB} & 47.78 (\dd) \\
\bottomrule
\end{tabular}
\label{tab.avmnist}
\end{center}
\end{table}

% \textbf{AV-MNIST classification} AV-MNIST \citep{} is an audio-visual dataset created from MNIST \citep{} and FSDD \citep{} dataset. Two modalities are vision (written digits) and audio (a human reading digits). Assume that we want to improve an audio model using KD. Unimodal KD resorts to a high-capacity audio model as the teacher while multimodal KD adopts an audio-visual teacher model. All other training configuration are identical. 

% \textbf{NYU Depth V2 Semantic Segmentation} NYU Depth V2 \citep{} contains 1449 densely labeled pairs of aligned RGB and depth images. Similarly, the goal is to improve an RGB model performance with KD. We experiment with using (1) a unimodal RGB teacher (2) a multimodal RGB-D teacher to train an RGB student model.

% \begin{table}[!h]
% \begin{center}
% \caption{Evaluation of unimodal distillation (UM-distill) and multimodal distillation (MM-distill) on AV-MNIST. Results are averaged over 10 runs.}
% \label{table:headings}
% \begin{tabular}{ccccc}
% \toprule
% Method & Teacher Modality & Teacher Acc (\%) & Student Modality & Student Acc (\%) \\
% \midrule
% No-distill & - & - & audio & 68.36 \\
% UM-distill & audio & 84.57 & audio & 70.10 \\
% MM-distill & image + audio & 91.61 & audio & 69.73 \\
% \bottomrule
% \end{tabular}
% \label{tab.avmnist}
% \end{center}
% \end{table}
\textbf{Failure Cases.} We provide two example failure cases of multimodal KD in Table \ref{tab.avmnist}. AV-MNIST \citep{avmnist} is an audio-visual dataset containing hand-written digits (\ie, grayscale images) and human speaking digits (\ie, audio). Here we attempt to improve an audio student using KD. NYU Depth V2 \citep{nyu} contains 1,449 pairs of aligned RGB and depth images. Similarly, the goal is to improve an RGB model performance with KD. Table \ref{tab.avmnist} reports a somewhat counter-intuitive finding: a more accurate multimodal network does not serve as a good teacher. Despite the great increase in teacher accuracy, multimodal KD fails to outperform unimodal KD. In the case of AV-MNIST, while the audio-visual teacher itself has a much higher accuracy than the unimodal teacher (\ie, +7.04\%), the resulting student is worse (\ie, -0.37\%) instead. Similarly, the great increase in teacher performance (\ie, +4.64\%) does not translate to student improvement (\ie, -0.22\%) on NYU Depth V2.

These results cast doubt on the efficacy of multimodal KD. Despite being more accurate, a multimodal network doesn't always teach a better student. Thus, contradictory to the previous intuition, teacher performance seems not reflective of student performance. Inspired by this observation, our work targets on exploring the open problem: \emph{What is the fundamental factor deciding the efficacy of multimodal KD?}

% \emph{If it is not related to the performance improvement brought by a multimodal teacher, what is the real decisive factor here?}


% In spite of the great empirical success reported in prior works \citep{}, we attempt to answer two fundamental questions: (1) \textit{Is multimodal KD always helpful?} (2) \textit{If not, what controls the effectiveness of multimodal KD?} 

% AV-MNIST common info small, because they are not paired.
% MM-IMDB common info large proportion




==> 3-2.method.tex <==
\newcommand{\df}{decisive features}
\newcommand{\gd}{general decisive features}
\newcommand{\sd}{specific decisive features}
\section{The Modality Focusing Hypothesis}\label{sec.hypothesis}
% If teacher performance does not tell us whether KD can help or not, what is the decisive factor that accounts for student performance in multimodal KD? 

% We now propose our explanations on the key ingredients determining the student performance in multimodal KD, which we termed as Modality Focusing Hypothesis (MFH) and built on the modality Venn Diagram.

% In addition, is there a way to improve performance for certain multimodal tasks?

\subsection{Modality Venn Diagram}\label{sec.venn}

In this section, we propose our model on the generating dynamics of multimodal data, termed as Modality Venn Diagram (MVD). For simplicity, we limit the number of modalities to two, denoted by modality $\{a,b\}$, respectively, and consider a $K$-class supervised classification task. Let $\mathcal{X}^a$, $\mathcal{X}^b$, and $\mathcal{Y}$ be the feature space of modality $a$, modality $b$, and the label space, respectively, and $(\mathbf{x}^a,\,\mathbf{x}^b,\,y)$ be a pair of data drawn from a unknown distribution $\mathcal{D}$ over the space $\mathcal{X}^a\times \mathcal{X}^b\times\mathcal{Y}$. MVD assumes that $(\mathbf{x}^a,\,\mathbf{x}^b,\,y)$ is generated by a quadruple $(\mathbf{z}^{sa},\,\mathbf{z}^{sb},\,\mathbf{z}^{0},y)\in\mathcal{Z}^{sa}\times\mathcal{Z}^{sb}\times\mathcal{Z}^0\times\mathcal{Y}$, following the generating rule: 
\begin{equation}
\begin{aligned}
\textsc{MVD Generation Rule:}\quad
&\mathbf{x}^a = \mathbf{g}^a(\mathbf{z}^{a}),\,&\mathbf{z}^a=[\mathbf{z}^{sa},\mathbf{z}^{0}]^T\in \mathcal{Z}^a=\mathcal{Z}^{sa}\times\mathcal{Z}^0\\
&\mathbf{x}^b = \mathbf{g}^b(\mathbf{z}^{b}),\,&\mathbf{z}^b= [\mathbf{z}^{sb},\mathbf{z}^{0}]^T \in \mathcal{Z}^b=\mathcal{Z}^{sb}\times\mathcal{Z}^0
\end{aligned}    
\end{equation}
where collectively, $g^u(\cdot):\mathcal{Z}^u\mapsto \mathcal{X}^u$ if we adopt the notation $u\in\{a,\,b\}$. To complete the MVD, another linear decision rule should be included. Specifically, the following equation:
\begin{equation}
\begin{aligned}
    \textsc{MVD Decision Rule:}\quad \exists\, \mathbf{w}^{u},\; &1[\mathbf{w}^{u,T}\mathbf{z}^u \geq 0]=y\\
\end{aligned}
\end{equation}
is assumed to hold for any $(\mathbf{z}^{sa},\,\mathbf{z}^{sb},\,\mathbf{z}^{0},y)$, where $1[\cdot]$ returns 1 if the argument is true and 0 otherwise. In essence, the two rules of MVD altogether specify that $\mathbf{x}^u$ is generated based on a \textit{modality-specific decisive feature} $\mathbf{z}^{su}$, and a \textit{modality-general decisive feature} $\mathbf{z}^0$. 

The proposed MVD model coincides with our common sense of multimodal data. Consider a video-audio data pair, as shown in Fig. \ref{fig.mod}, where the camera only captures one person due to its position angle and the audio is mixed sounds of two instruments. The true label ``playing instruments'' can be correctly inferred with three sources of information: visual \sd, audio \sd \ and modality-general decisive features. 

We now informally touch our Modality Focusing Hypothesis (MFH), and provide a theoretical guarantee in an analytically tractable case, linear binary classification. Let $\mathcal{Z}^{su}\subseteq\mathbb{R}^{d_{su}}$ and $\mathcal{Z}^0\subseteq\mathbb{R}^{d_0}$, so that $\mathcal{Z}^u\subseteq\mathbb{R}^{d_u}$, where $d_u=d_{su}+d_0$. For later simplicity, we denote a ratio $\gamma=d_0/(d_0+d_{sa}+d_{sb})\in[0,1]$. As an illustrating example, consider both $\mathbf{g}^a(\cdot)$ and $\mathbf{g}^b(\cdot)$ are identity function.
Our intuition is that, as $\gamma$ gradually increases from $0$ to $1$, transferring the knowledge from a teacher $\mathbf{f}_{\bm{\theta}_t}(\cdot):\mathcal{X}^a\mapsto\mathcal{Y}$ to a student $\mathbf{f}_{\bm{\theta}_s}(\cdot):\mathcal{X}^b\mapsto\mathcal{Y}$ should become easier. Because (i) the feature $\mathbf{x}^a$ and $\mathbf{x}^b$ have more overlapping, and (ii) the non-overlapping parts do not have the capability to represent each other \footnote{To support this claim, as shown in Fig.~\ref{fig.mod}, how could a picture of the left person represent the sound of the instrument in the hand of the right person?}. Same intuition applies to the case when $\mathbf{g}^a(\cdot)$ and $\mathbf{g}^b(\cdot)$ are complicated real multi-dimensional functions. Formally, considering an infinitesimal learning rate which turns the training into a continuous gradient flow defined on a time parameter $t\in[0,\+\infty)$~\citepp{phuong2019towards}, if $n$ data are available, which are collectively denoted as $\mathbf{Z}^{u}\in\mathbb{R}^{d_u\times n}$, we have the following theorem to bound the training distillation loss using the value of $\gamma$ in a linear binary classification.

\begin{theorem}\label{thm:cmd_linear_binary}
(Crossmodal distillation in linear binary classification). Without loss of generality, we assume $\mathbf{f}_{\bm{\theta}_t}(\cdot):\mathcal{X}^a\mapsto\mathcal{Y}$ and  $\mathbf{f}_{\bm{\theta}_s}(\cdot):\mathcal{X}^b\mapsto\mathcal{Y}$.
Suppose $\max\{||\mathbf{Z}^u\mathbf{Z}^{u,T}||,\,||(\mathbf{Z}^u\mathbf{Z}^{u,T})^{-1}||\}\leq\lambda$ always holds for both $u=a$ or $b$, and $\mathbf{g}^u(\cdot)$ are identity function. If there exists $(\epsilon, \delta)$ such that
\begin{equation}
    \text{Pr}\left[||\mathbf{Z}^{a,T}\mathbf{Z}^{a}-\mathbf{Z}^{b,T}\mathbf{Z}^{b}||\leq (1-\gamma)\epsilon\right]\geq 1-\delta
\end{equation}
Then, with an initialization at $t=0$ satisfying $R_n^{\text{dis}}(\bm{\theta}_s(0))\leq q$,  we have, at least probability $1-\delta$:
\begin{equation}
    R_n^{\text{dis}}(\bm{\theta}_s(t=+\infty)) \leq n (\frac{\epsilon^\star}{1-e^{-\epsilon^\star}}-1-\ln{\frac{\epsilon^\star}{1-e^{-\epsilon^\star}}}) 
\end{equation}
where $\epsilon^\star=\lambda^{1.5}(\lambda^2+1)(1-\gamma)\epsilon$ and $R_n^{\text{dis}}(\bm{\theta}_s)$ is the empirical risk defined by KL divergence:
\begin{equation}
\begin{aligned}
R_n^{\text{dis}}(\bm{\theta}_s(t))=&\sum_{i=1}^n -\sigma(\bm{\theta}_t^T\mathbf{x}^a_i)\cdot\ln\frac{\sigma(\bm{\theta}_s^T\mathbf{x}^b_i)}{\sigma(\bm{\theta}_s^T\mathbf{x}^a_i)}-\left[1-\sigma(\bm{\theta}_t^T\mathbf{x}^a_i)\right]\cdot\ln\frac{1-\sigma(\bm{\theta}_s^T\mathbf{x}^b_i)}{1-\sigma(\bm{\theta}_s^T\mathbf{x}^a_i)}
\end{aligned}
\end{equation}
\end{theorem}

The proof is postponed till the appendix.

\textbf{I am a separating line.}

%To study multimodal KD, it is critical to first establish an understanding of multimodal data. We propose the modality Venn diagram that depicts the relationship between two modalities in Figure \ref{fig.mod}. The diagram reflects the common perception that multimodal data possess shared information and preserve information specific to each modality as well \citep{}. Following a causal perspective \citep{} (\ie, features cause labels), we assume that label $\mathbf{y}$ is determined by a subset of features; this subset of features are referred to as \emph{decisive features} throughout the paper. For instance, color features of an image help identify the correct class for this image and can be considered as \df. 

To study multimodal KD, it is critical to first establish an understanding of multimodal data. But before touching multimodal data, let us first fall back and consider unimodal data. Following a causal perspective \citep{scholkopf2012causal,lopez2015unifying} (\ie, features cause labels), we assume that the label $\mathbf{y}$ is determined by a subset of features in $\mathbf{x}_1$ (or $\mathbf{x}_2$); this subset of features are referred to as \emph{decisive features} for modality 1 (or modality 2) throughout the paper. For instance, colors of an image help identify some classes (\eg, distinguish between a zebra and a horse) and can be considered as \df. 

When considering multimodal data, input features of the two modalities will have logical relations such as intersection and union. To capture this relationship, we propose the modality Venn diagram in Fig. \ref{fig.mod}. The diagram reflects the common perception that multimodal data possess shared information and preserve information specific to each modality as well \citep{wang2016learning,zhang2018multimodal,hazarika2020misa}. Decisive features of the two modalities are thus composed of two parts: (1) \emph{modality-general decisive features} (colored in dark purple) and (2) \emph{modality-specific decisive features} (colored in light purple). Consider a video-audio data pair, as shown in Fig. \ref{fig.mod}, where the camera only captures one person due to its position angle and the audio is mixed sounds of two instruments. The true label ``playing instruments'' can be correctly inferred with three sources of information: visual \sd, audio \sd \ and modality-general decisive features. Fig. \ref{fig.mod} left illustrates how we interpret these three sources of information at the input level. 

% Consider an image-audio data pair, as shown in Fig. \ref{fig.mod} right, the label can be correctly inferred with three sources of information, a barking dog (\ie, \gd), a dog tail (\ie, \sd \ in the visual modality) and a dog sound (\ie, \sd \ in the audio modality).

To quantify the relative importance of these three features, we define $\gamma$, $\alpha_1$ and $\alpha_2$ as follows. Let $\gamma$ be the relative importance of \gd \ among all \df. $\alpha_1$ and $\alpha_2$ denote the relative importance of \sd \ in modality $1$ and $2$, respectively. There are multiple ways to calculate the relative importance, and we discrete input features by assigning a binary label for each feature dimension (\ie, this dimension belongs to \gd \ or \sd). The ratio of general decisive feature channel number to decisive feature channel number approximates $\gamma$. $\alpha_1$ and $\alpha_2$ are calculated in a similar way, and we have $\alpha_1+\alpha_2+\gamma=1$.

 \begin{figure}[!h]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/modvenn_v1.png}
    \caption{Left: an input video-audio pair can be regarded as composed of modality general features and modality-specific features in the visual and audio modality. For instance, the man playing violin in the right is not captured by the camera and hence its sound (colored in pink) belongs to audio modality-specific information. Those three parts of features work together and contribute to the final label $\mathbf{y}$. Right: the modality Venn diagram. For any given pair of multimodal features (input-level, middle-level, output-level), there exist \gd \ (colored in dark purple) and \sd \ (colored in light purple).}
    \label{fig.mod}
\end{figure}
% Right: True label is caused by multimodal decisive features, which consist of \gd \ and \sd \ in the visual and audio modality.
% First, we present an understanding of multimodal data using Venn Diagram. We adopt a causal perspective \citep{}, \ie, assume that the features cause the labels. Following the previous notation, we denote input data with two modalities as $(\mathbf{x}_1, \mathbf{x}_2)$. Let $\mathbf{y}$ represent the ground truth label and $\mathbf{x}^*$ be the privileged multimodal features (we define privileged features as features that directly cause the label). As depicted in Figure \ref{fig.Venn}, $\mathbf{x}^*$ consists of modality-general features as well as modality-specific features extracted from $(\mathbf{x}_1, \mathbf{x}_2)$ and cause label $\mathbf{y}$. Let $\alpha$, $\beta$ and $\gamma$ represent the ratio of modality-specific ($\mathbf{x}_1$), modality-specific ($\mathbf{x}_2$) and modality-general privileged features over all privileged features, respectively. $\alpha + \beta + \gamma = 1$.

% The core idea is that multimodal data possess shared information (described by $\mathbf{x}_1 \cap \mathbf{x}_2$) and preserve information specific to each modality as well. We assume that these two sources of information work together to determine the final label $\mathbf{y}$; this assumption is widely adopted and motivates the design of many multimodal networks \citep{}. 

% this is a generalized version of the conditional independence assumption \citep{} in multimodal learning. Moreover, this assumption is also commonly perceived and motivates the design of many fusion models \citep{}.

% Label $y$ is determined by privileged modality-general features (colored in dark red) and modality-specific features (colored in pink). Based on this understanding, we 


Now we are ready to consider crossmodal KD (\ie, $\mathbf{x}_T\leftarrow\mathbf{x}_2$, $\mathbf{x}_S\leftarrow\mathbf{x}_1$). Clearly, teacher performance is controlled by both \gd \ and \sd \ in modality $2$. However, we find that: (i) Although \sd \ in modality $2$ are meaningful for the teacher, they can not instruct the student since the student only sees modality $1$; (ii) On the other hand, \gd \ are not specific to modality $2$ and could be transferred to the student. This motivates our modality focusing hypothesis.

% Therefore, the role of crossmodal KD is to assist the student network in learning \gd.

\textbf{The Modality Focusing Hypothesis.} \emph{In multimodal KD and crossmodal KD (defined in Sec. \ref{sec.problem}), distillation performance is dependent on \gd \ in the teacher network: with larger $\gamma$, the student network is expected to perform better.} 

% (1) For crossmodal KD, a $\mathbf{x}_2$ model that focuses more on GD features functions as a better teacher; (2) For multimodal KD, a multimodal network that focuses less on SD features in modality $2$ is a better teacher.

% Based on this understanding, we present the Modality Focusing Hypothesis. Consider the distillation where the teacher takes $\mathbf{x}_2$ as input and the student takes $\mathbf{x}_1$ as input, as shown in Figure \ref{} (c). Clearly, teacher and student performance is determined by $\beta+\gamma$ and $\alpha+\gamma$, respectively. Crossmodal distillation enables the teacher to transfer knowledge about modality-general features ($\gamma$) to the student, but can not help the student better extract modality-specific features ($\alpha$). Consequently, the student can better ``focus'' on modality-general features, and is thus beneficial for the case where $\gamma$ is large (\ie, multimodal data share many label-relevant information). To conclude, distillation performance is directly related to $\gamma$: with larger $\gamma$ (smaller $\alpha$ and $\beta$), the student is expected to perform better.

% In our hypothesis, the amount of modality-general information (\ie, $\gamma$) is what really influences multimodal distillation performance. 

% also provides a good illustration of the problem and facilitates our understanding for real multimodal applications.

The hypothesis states that in multimodal knowledge transfer, the student learns to ``focus on'' \gd. Multimodal KD is thus beneficial for the case where $\gamma$ is large (\ie, multimodal data share many label-relevant information). Moreover, this poses a valid explanation for the observation in Sec. \ref{sec.failurecase}. Since teacher performance is influenced by \df \ while student performance is only related to \gd, it is plausible that teacher performance fails to correlate with student performance in some scenarios. For instance, when $\alpha_2$ is large and $\gamma$ is small, the teacher network attains high accuracy primarily based on modality-specific information, which is not visible to the student. In such case, we may find that a high-accuracy teacher does not lead to a good student.


% To verify the hypothesis, we first experiment with synthetic Gaussian data; this example provides a good illustration of when multimodal KD is effective, and when it is not. We generate multimodal data $(\mathbf{x}_1, \mathbf{x}_2)$, with $\mathbf{x}_1$ and $\mathbf{x}_2$ randomly sampled from two Gaussian distributions. Details of data generation can be found in Sec. \ref{}. Starting from the extreme case where two modalities do not overlap (\ie, $\gamma=0$), we gradually increase the proportion of \gd \ until all \df \ are shared by two modalities (\ie, $\gamma=1$), as illustrated in Figure \ref{fig.gaussb1}. We plot the accuracy of the teacher, student and a regularly-trained student without distillation as the student baseline during this process. 
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.9\linewidth]{figs/gaussb1.pdf}
    \caption{An illustration of the modality focusing hypothesis with synthetic Gaussian data. Teacher modality is $\mathbf{x}_2$ and student modality is $\mathbf{x}_1$. We plot the confidence interval of one standard deviation for student accuracy. With increasing $\gamma$, crossmodal KD becomes more effective.}
    \label{fig.gauss1}
\end{figure}

To have an intuitive and quick understanding of our hypothesis, here we show an experiment with synthetic Gaussian data. More details can be found in Sec. \ref{sec.expgauss}. As shown in Fig. \ref{fig.gauss1}, we start from the extreme case where two modalities do not overlap, and gradually increase the proportion of \gd \ until all \df \ are shared by two modalities. We observe that crossmodal KD fails to work when $\mathbf{x}_1$ and $\mathbf{x}_2$ share few \df \ (\ie, $\gamma$ is small) as \sd \ in modality $2$ are not perceived by the student. As $\gamma$ gradually increases, crossmodal KD becomes more effective. For the case where all \df \ possess in both modalities, the student benefits from teacher's knowledge on \gd \ and outperforms its baseline by 2.1\%. Note that the teacher accuracy does not vary much during this process, yet student performance differs greatly. This further lends support to our hypothesis and demonstrates that teacher accuracy does not faithfully reflect the effectiveness of crossmodal KD. 

% Apart from varying $\gamma$, we also conduct experiments with varying $\alpha_1$, $\alpha_2$ and other variables to provide a comprehensive analysis in Sec. \ref{sec.expgauss} and Appendix.  

% Without loss of generality, we always assume student only takes input data from modality $1$. 
% with $\mathbf{x}_1$ and $\mathbf{x}_2$ being a 50-dimension and 25-dimensional vector.

% We observe improved student performance with increasing $\gamma$. For case (a), where $\mathbf{x}_1$ and $\mathbf{x}_2$ do not share any \df, crossmodal KD fails to work and results in a student with 2.98\% lower accuracy compared with the baseline. For case (b), where all \df \ possess in both modalities, crossmodal KD becomes effective and improves student accuracy by 3.13\%. Note that the teacher accuracy does not vary much during this process, yet student performance differs greatly. This further supports our hypothesis and demonstrates that teacher accuracy does not indicate the effectiveness of multimodal KD. Apart from varying $\gamma$, we also conduct experiments with varying $\alpha_1$, $\alpha_2$ and other variables to provide a comprehensive analysis in Sec. \ref{sec.expgauss} and Appendix. 

The modality focusing hypothesis offers a new perspective to understand multimodal KD. Below we describe one important implication to showcase its practical value. 

\textbf{Implication.} For multimodal KD (crossmodal KD), consider two teachers with identical architectures: Teacher (a) makes predictions primarily based on \gd \ while teacher (b) relies more on modality-specific information. In other words, teacher (a) has a larger $\gamma$ than teacher (b). \emph{We expect that the student taught by teacher (a) yields better performance than that by teacher (b).}

By drawing inspiration from the implication, we can train a teacher network that ``focuses on'' \gd \ for prediction. Compared with a regularly-trained teacher, the new teacher is tailored for distillation task and can possibly lead to a better student. The modality focusing hypothesis equips us with a new type of approaches to improve multimodal KD. 

\subsection{Modality-General Decisive Feature Separation}

% \Gao{most important, please check the use of words general decisive, decisive, modality-general decisive, etc., making sure they are used correctly at the right place}

In the synthetic Gaussian case, we set up the experiment by manually controlling \gd. However, in real multimodal datasets, modality-general decisive features are unknown and need to be identified. Here we propose a permutation-based approach to address this problem.


% We have presented the modality focusing hypothesis and validated it on synthetic data. Next, we aim to verify the hypothesis on real multimodal data. Since we cannot directly acquire \gd \ from real data, it is necessary to adopt a pre-processing step to extract these features from multimodal data. 

The major steps of our proposed method are demonstrated in Algorithm \ref{alg.sep}. The input of Algorithm \ref{alg.sep} are $\mathbf{X}_1 \in \mathbb{R}^{N\times D_1}$, $\mathbf{X}_2 \in \mathbb{R}^{N\times D_2}$, and $\mathbf{Y}\in\mathbb{R}^N$, representing $N$ paired features from modality $1$ and $2$, and $N$ target labels, respectively. The output is a saliency vector $\mathbf p \in \mathbb{R}^{D_2}$ for \gd \ in modality $2$, where its $d$-th entry $p_d \in \left[0, 1\right]$ reflects the saliency of the $d$-th feature dimension. A larger saliency value indicates a more general decisive feature channel.

\begin{algorithm}
\caption{Modality-General Decisive Feature Separation}\label{alg.sep}
\begin{algorithmic}[1]
\Require {multimodal data $(\mathbf{X}_1 \in \mathbb{R}^{N\times D_1},\mathbf{X}_2 \in \mathbb{R}^{N\times D_2},\mathbf{Y}\in\mathbb{R}^N)$} 
\Ensure saliency vector $\mathbf{p} \in \mathbb{R}^{D_2}$ for features of modality $2$
\State Jointly train two unimodal networks $\mathbf{f}_{\boldsymbol{\theta}_1^*}$ and $\mathbf{f}_{\boldsymbol{\theta}_2^*}$ using the following loss:
 \begin{equation}
   \min_{\boldsymbol{{\theta}_1}, \boldsymbol{{\theta}_2}} \mathcal L = Dist(\mathbf{f}_{\boldsymbol{\theta}_1}(\mathbf{X}_1), \mathbf{f}_{\boldsymbol{\theta}_2}(\mathbf{X}_2)) + CE(\mathbf{Y}, \mathbf{f}_{\boldsymbol{\theta}_1}(\mathbf{X}_1)) + CE(\mathbf{Y}, \mathbf{f}_{\boldsymbol{\theta}_2}(\mathbf{X}_2))
   \label{eq.train}
\end{equation}
\Comment {$Dist(\cdot,\cdot)$ denotes a distance loss (\eg, mean squared error)}
\For{$d = 1$ to $D_2$}\Comment{Calculate the saliency for the $d$-th feature dimension}
  \State $p_d = 0$
  \For{$k = 1$ to $K$}\Comment{Repeat permutation $K$ times for better stability}
        \State {permute the $d$-th column of $\mathbf{X}_2$ yielding $\mathbf{\tilde X}_2$}
        \State {$p_d = p_d + \frac{1}{K}\times Dist(\mathbf{f}_{\boldsymbol{\theta}_1^*}(\mathbf{X}_1), \mathbf{f}_{\boldsymbol{\theta}_2^*}(\mathbf{\tilde X}_2))$}
    \EndFor
\EndFor
\State Perform normalization: $\mathbf{p} = \frac{\mathbf{p}}{\max_d{p_d}}\in [0,1]^{D_2}$
\end{algorithmic}
\end{algorithm}

% We present two steps to detach \gd \ for modality $2$ in Algorithm \ref{alg.sep}. The approach is similar for modality $1$. Let $\mathbf{X}_1 \in \mathbb{R}^{N\times D_1}$ denote $N$ input data from modality $1$, where the $i$-th row denotes $i$-th training data (a $D_1$-dimensional vector). $\mathbf{X}_2 \in \mathbb{R}^{N\times D_2}$ denotes $N$ data from modality $2$, and each input vector is of dimension $D_2$. The output is a saliency vector $\mathbf p \in \mathbb{R}^{D_2}$, where $p_i \in \left[0, 1\right]$ reflects the saliency of \gd \ in dimension $i$. A larger value indicates that the corresponding dimension is more ``general decisive''. 

\textbf{Clarifications.} Inspired by the fact that input-level features contain much label-irrelevant noise, as shown in the right of Fig. \ref{fig.mod}, our Algorithm \ref{alg.sep} is designed following a trace-back thought starting from the output level. Namely, we drive two unimodal networks to the state of ``feature alignment'' at the output level using Eq. (\ref{eq.train}), and then use permutation to identify which input feature dimension has a larger impact to the state. Those more influential to the state (\ie, a large distance in step 6) will be assigned a larger saliency value.

In step 1, we jointly train two unimodal networks $\mathbf{f}_{\boldsymbol{\theta}_1^*}$ and $\mathbf{f}_{\boldsymbol{\theta}_2^*}$ that respectively take unimodal data $\mathbf{X}_1$ and $\mathbf{X}_2$ as input. The first loss term in Eq. (\ref{eq.train}) aims to align feature spaces learned by the two networks, and the remaining loss terms ensure that learned features are essential for a correct prediction. We believe that this training strategy aligns three sources of \df \ at the output level. In step 2, we follow the idea of permutation feature importance~\citep{breiman2001random} to trace back \gd \ at the input level. For the $d$-th dimension in $\mathbf{X}_2$, we randomly permute $\mathbf{X}_2$ along this dimension and obtain a permuted $\mathbf{\tilde X}_2$ in step 5. Next, we calculate the distance between $\mathbf{f}_{\boldsymbol{\theta}_1^*}(\mathbf{X}_1)$ and $\mathbf{f}_{\boldsymbol{\theta}_2^*}(\mathbf{\tilde X}_2)$ in step 6. A large distance indicates that the $d$-th dimension largely influences the state of ``feature alignment''. Consequently, we are able to quantify the relative importance of each input feature channel and use the saliency vector $\mathbf{p}$ to represent it. We repeat the permutation process for $K$ times and average the distance value for good stability. Finally, $\mathbf{p}$ is normalized to $[0,1]^{D_2}$ in step 9.

% \Xue{Need some discussion} We believe that with only the last two cross entropy terms, the modality Venn diagram looks like that at the output level in the left of Fig. \ref{fig.mod}. However, with the additional first distance loss, the middle region marked by $\gamma$ expands to engulf the peripheral light red regions marked by $\alpha_1$ and $\alpha_2$.
% While the final goal is to separate \df \ from $\mathbf{X}_2$, input data contain much label-irrelevant noise, as shown in Figure \ref{fig.mod} left. Therefore, we start with feature separation at the output level, where all features contribute to the final label and can be considered as \df. In the first step, we jointly train two unimodal networks $\mathbf{f}_{\boldsymbol{\theta}_1}$ and $\mathbf{f}_{\boldsymbol{\theta}_2}$ that respectively take unimodal data $\mathbf{X}_1$ and $\mathbf{X}_2$ as input, as in Eq. (\ref{eq.train}). The first loss term aims to align feature spaces learned by the two networks, and the remaining loss terms ensure that learned features are essential for a correct prediction. 

% After training, we obtain trained models $\{\boldsymbol{\theta}_1^*, \boldsymbol{\theta}_2^*\}$ and derive features at the output level. In the next step, we follow the idea of permutation invariance \citep{} to trace back \gd \ at the input level. For each dimension in $\mathbf{X}_2$, we randomly permute $\mathbf{X}_2$ along this dimension and obtain a permuted $\mathbf{\tilde X}_2$. Output features in modality $1$ (\ie, $\mathbf{f}_{\boldsymbol{\theta}_1^*}(\mathbf{X}_1)$) are considered as a baseline. We compare the distance between output features with permuted $\mathbf{\tilde X}_2$ being the input (\ie, $\mathbf{f}_{\boldsymbol{\theta}_2^*}(\mathbf{\tilde X}_2))$ and the baseline. A large distance indicates that this dimension largely influences the final \gd. Consequently, we are able to quantify the relative importance of each input feature channel and use the saliency vector $\mathbf{p}$ to represent it. We repeat the permutation process for $K$ times and average the distance value. Finally, $\mathbf{p}$ is normalized between 0 and 1.

% Based on the Modality Venn Diagram, the privileged modality-general features are shared by two modalities and indicate label $\mathbf y$. We give the definition for a set of functions $(\mathbf{f}_1, \mathbf{f}_2)$ that extracts privileged modality-general features:

% \begin{equation}
%     \{(\mathbf{f}_1, \mathbf{f}_2)| \mathbf{h}_{com} = \mathbf{f}_1(\mathbf{x}_1) = \mathbf{f}_2(\mathbf{x}_2), \argmax(\mathbf{h}_{com}) =\mathbf y, \forall {(\mathbf{x}_1, \mathbf{x}_2)} \}
%     \label{eq.def}
% \end{equation}
% Here $\mathbf{f}_1$ and $\mathbf{f}_2$ map input data $\mathbf{x}_1$ and $\mathbf{x}_2$ to shared features $\mathbf{h}_{com}$, respectively. $\mathbf{h}_{com}$ contains modality-invariant information and is predictive of true label $\textbf{y}$, and thus represents the privileged modality-general features. 

% In practice, we realize $\mathbf{f}_1$ and $\mathbf{f}_3$ to be one neural network, where $\mathbf{f}_1$ is the first few layers (\ie, feature extraction block) and $\mathbf{f}_3$ corresponds to the remaining layers (\ie, linear projection block). $\mathbf{f}_2$ functions similarly as $\mathbf{f}_1$, but takes $\textbf{x}_2$ as input.

% Following the definition above, we jointly optimize $\mathbf{f}_1$ and $\mathbf{f}_2$ to obtain the desired $\mathbf{h}_{com}$. The loss term is shown below:
% \begin{equation}
%     \mathcal L = Dist(\mathbf{f}_1(\mathbf{x}_1), \mathbf{f}_2(\mathbf{x}_2)) + CE(\mathbf{y}, \mathbf{f}_1(\mathbf{x}_1)) + CE(\mathbf{y}, \mathbf{f}_2(\mathbf{x}_2))
% \end{equation}
% where $Dist$ denotes a distance loss (\eg, mean squared error). The first loss pushes hidden representations of $\mathbf{x_1}$ and $\mathbf{x_2}$ closer and the other two terms ensure that the extracted features are essential for a correct prediction.

% After training, we obtain models $\mathbf{f}^*_1$ and $\mathbf{f}^*_2$. $\mathbf{h}_1 = \mathbf{f}^*_1(\mathbf{x}_1)$ and $\mathbf{h}_2 = \mathbf{f}^*_2(\mathbf{x}_2)$ are close approximations of $\mathbf{h}_{com}$ defined in Eq. (\ref{eq.def}). Now that we have identified $\mathbf{h}_{com}$ at the output level, we aim to further  separate privileged modality-general features at the input level and propose an approach based on permutation invariance \citep{}. 

% Let $\mathbf{X}^1 \in R^{N\times D_1}$ denote $N$ input data from modality $1$, where each row $\mathbf{x}^1 \in R^{1\times D_1}$ is a $D_1$-dimensional vector. Similarly, $\mathbf{X}^2 \in R^{N\times D_2}$. Algorthm \ref{} describes steps to detach modality-general feature channels for modality $1$: for each feature dimension, we randomly permute $\mathbf{X}^1$ along that dimension and calculate the differences between outputs. This measures how critical a dimension is for privileged modality-general features. The returned vector $\mathbf{z} \in R^{D_1}$ quantifies how `privileged modality-general' each feature dimension is, where $z_i$ reflects the amount of privileged modality-general information for the $i$-th feature channel in $\mathbf{X}_1$. A large value corresponds to more privileged modality-general information and a small value indicates modality-specific or non-privileged information. The procedure to separate privileged modality-general features in $\mathbf{X}^2$ is similar.

\textbf{Remarks.} First, Algorithm \ref{alg.sep} is not limited to feature separation at the input level. $\mathbf{X}_1$ and $\mathbf{X}_2$ can be features extracted from middle layers of the neural network as well. In such case, output $\mathbf{p}$ reflects the saliency of \gd \ for each middle-layer feature channel. Secondly, based on $\mathbf p$, we can decide whether each input dimension is ``general decisive'' or ``non general decisive''. For instance, we can set a hard threshold or pick a certain ratio according to sorted $\mathbf p$. This provides us with a way to control $\gamma$ for a given teacher network. In the experiments (Sec. \ref{sec.exp}), we nullify general decisive or non general decisive feature channels identified by  Algorithm \ref{alg.sep} to obtain teacher models with different $\gamma$ to justify the hypothesis. Last but not least, Algorithm \ref{alg.sep} could be equally applied to identify modality-general decisive features for modality $1$ as long as we permute $\mathbf{X}_1$.

% Thus, $\gamma$ can be calculated as the ratio of general decisive feature number to $D_2$.

% First, the design intention of our Algorithm \ref{alg.sep} is based on the two ideas: (i) drive the two unimodal networks to a state which could represent modality-general decisive feature separation, and (ii) identify the impact of each input feature dimension to the state using permutation. The key is a good loss capturing the state that could be put at the place of Eq. (\ref{eq.train}). Our current choice is a distance loss plus two classification losses.

% Here we present a general approach to separate \gd \ from any given multimodal features. The application may go beyond verifying our modality focusing hypothesis. We hope this can facilitate multimodal understanding and help inspire related multimodal research as well.

% \subsection{Implications Derived from the Hypothesis}\label{sec.implication}
% alternative title: Make Multimodal Distillation Efficient,  distillation guidance, guide multimodal distillation, 

% The modality focusing hypothesis and modality-general decisive feature separation method provide a new perspective to understand multimodal KD. In this section, we discuss two important implications to showcase their practical value. 

% Without loss of generality, we always assume student only takes input data from modality $1$. 

% \textbf{Implication I:} For crossmodal KD, consider two teacher networks with identical architectures taking input data from modality $2$; Teacher (a) makes predictions primarily based on \gd \ while teacher (b) relies more on \sd. In other words, teacher (a) has a larger $\gamma$ (smaller $\alpha_2$) than teacher (b). \emph{We expect that the student taught by teacher (a) yields better performance than that by teacher (b).}

% \textbf{Implication II:} For multimodal KD, consider two teachers with identical network architectures taking input data from both modality $1$ and $2$; Teacher (a) has a smaller $\alpha_2$ (larger $\alpha_1 + \gamma$) than teacher (b). \emph{The student taught by teacher (a) is expected to perform better than that by teacher (b).}


% \textbf{Implication (1)} For crossmodal KD, consider two teacher networks with identical architectures; the unimodal teachers extract \gd \ and \sd \ in modality 2. Teacher network (a) makes predictions primarily based on \gd \ while teacher network (b) relies more on \sd. In other words, teacher (a) has a larger $\gamma$ (smaller $\alpha_2$) than teacher (b). We expect that the corresponding student network (a) yields better performance than student network (b). 

% The Feature Separation method enables us to verify the Modality Focusing hypothesis for real multimodal data. To be specific, we first classify input features as `privileged modality-general' or `non privileged modality-general'. Next, we remove `privileged modality-general' and `non-privileged modality-general' features for modality $2$ and compare results on crossmodal distillation. We expect that removing `non-privileged modality-general' features in $\mathbf{x}_2$ does not influence student performance while removing `privileged modality-general' features is likely to decrease student performance. For both cases, the teacher performance is expected to drop. The experimental results are presented in Section {} and aligns with our hypothesis: teacher accuracy is not correlated with distillation performance. Our proposed $\gamma$ is the decisive factor.  

% remove modality-specific features in teacher, teacher ↓, student ↑/-. remove modality-common features in teacher, teacher ↓, student ↓.

% This shows that teacher accuracy is not necessarily correlated with distillation performance. Our proposed alpha / beta is key.

% \textbf{Implication (2)} For multimodal KD, consider two teachers with identical network architectures; the multimodal teachers extract \gd \ and \sd \ from both modalities. If teacher (a) has a smaller $\alpha_2$ (larger $\alpha_1 + \gamma$) than teacher (b), student (a) is expected to perform better than student (b). 

% To best utilize a multimodal teacher, it is suggested to train a teacher that ``focuses on'' privileged modality-general features. Compared with a naive multimodal teacher, the new teacher benefits from the Modality Focusing Hypothesis and can lead to better distillation performance.

% In distillation task, train a teacher that focuses on common features. Compared with a naive teacher, the new teacher can lead to better distillation performance.

==> 4.exp.tex <==
\section{Experimental Results}\label{sec.exp}
To justify the modality focusing hypothesis, we design two sets of experiments: (1) For synthetic data, we can control its inherent characteristics (\ie, $\alpha_1$, $\alpha_2$ and $\gamma$) and perform KD. We are curious whether teacher and student performance are as described in the modality focusing hypothesis. Meanwhile, we report the accuracy of our Algorithm \ref{alg.sep} since 
whether a feature channel is general/specific decisive is known. (2) For real-world data, we cannot know the ground truth $\gamma$. To evaluate the implication in Sec. \ref{sec.venn}, we experiment with a modality-general teacher and a modality-specific teacher (\ie, one teacher with a large $\gamma$ and one teacher with a small $\gamma$). The two teachers can be obtained by applying Algorithm \ref{alg.sep} to estimate $\mathbf{p}$ and then removing corresponding feature channels in the teacher (Sec. \ref{sec.expravdess} and Sec. \ref{sec.expvgg}). Alternatively, we can apply specific training techniques to obtain a modality-general teacher (Sec. \ref{sec.expnyu}). In all, we provide experiments on 6 datasets (synthetic Gaussian, AV-MNIST, RAVDESS, VGGSound, NYU Depth and MM-IMDB) with diverse modalities (\ie, RGB images, depth images, audio and text). Due to space limit, some results (\eg, experiments on MM-IMDB~\citep{imdb} movie genre classification) and ablation studies are presented in the Appendix.
% Therefore, we adopt Algorithm \ref{alg.sep} to identify \gd. Based on estimated $\mathbf{p}$, we experiment with a modality-general teacher and a modality-specific teacher to evaluate the two implications in Sec. \ref{sec.implication}. 


% (1) We vary $\alpha_1$, $\alpha_2$ and $\gamma$ in multimodal data and observe teacher and student performance. (2) Given multimodal data, we calculate the saliency vector $\mathbf{p}$ with Algorithm \ref{alg.sep} and compare it with ground truth. (3) We evaluate the two implications in Sec. \ref{sec.implication} by experimenting with different teacher networks for distillation. For instance, we can remove non modality-general decisive feature channels identified by Algorithm \ref{alg.sep} and obtain a new teacher that focuses on \gd. Then we compare student performances corresponding to different teacher networks.

% While the first and second experiment directly support the modality focusing hypothesis and modality-general decisive feature separation method, they can only be evaluated on synthetic data since real-world multimodal data distribution (\ie, the value of $\alpha_1$, $\alpha_2$ and $\gamma$) is unknown. The last set of experiments is conducted on 5 real-world multimodal datasets with diverse modality combinations to demonstrate how the proposed hypothesis can benefit multimodal KD (crossmodal KD) and lead to performance improvement.


\subsection{Synthetic Gaussian}\label{sec.expgauss}

% We have presented the experiment with increasing $\gamma$ in Sec. \ref{sec.venn}. The experimental setting is as follows: $D_1=50, D_2=25, D=20$, we gradually increase $|J_1\cap J_2|$ from 0 to 10, with a step size of 2 and perform KD on every step. $\boldsymbol{\beta}$ is sampled from the standard normal distribution. Teacher and student are logistic regression models. There are 200 training data and 1000 test data. Furthermore, we experiment with increasing $\alpha_2$. Let $D_1=D_2=50$ and $D=|J_1\cup J_2|$ vary from 10 to 50. Fig. \ref{} below illustrates the process where modality-specific decisive features in modality $2$ gradually dominate. With increasing $\alpha_2$ (\ie, decreasing $\gamma$), the teacher gradually improves since it receives more modality-specific decisive features for prediction. However, the student network fails to benefit from the improved teacher and performs slightly worse instead. These results support our proposed modality focusing hypothesis:  teacher performance is not reflective of student performance. It is the amount of modality-general decisive information that matters. This set of experiment offers a valid explanation about the failure of multimodal KD.

% kd loss ratio

% Fig. \ref{fig.gaussb1} indicates that student performance is controlled by $\gamma$, rather than teacher accuracy. 

Next, based on the saliency vector $\mathbf{p}$ given by Algorithm \ref{alg.sep}, we identify feature channels that correspond to non modality-general decisive features and remove them in $\mathbf{X}_2$ to form a ``clean'' version of data that only contains \gd, $\mathbf{\hat X}_2$. We train a new teacher model with $\mathbf{\hat X}_2$ and apply KD subsequently. The new teacher is more modality-general compared with the regularly-trained teacher. We experiment with different values of $\gamma$ and summarize the results in Table \ref{tab.gauss}. Results are averaged over 10 runs.

% \begin{table}[!h]
% \begin{center}
% \caption{Evaluation on Gaussian data. FS Acc. denotes the accuracy of our feature separation method for $\mathbf{X}_2$. T and S represent teacher and student network, respectively.}
% \begin{tabular}{cc|ccc|c|ccc}
% \toprule
% \multirow{2}{*}{$\gamma$} & \multirow{2}{*}{\makecell[c]{FS\\Acc.}} & \multicolumn{7}{c}{Accuracy (\%)}\\
%  & & T & Modified T & $\Delta$ & S baseline & S & Modified S & $\Delta$ \\
% \midrule
% % 0.25 & 0.90 & 89.70 & 64.84 & \dd24.86 & 59.29 & 59.46 & 61.01 & \uu 1.55\\
% 0.33 & 0.98 & 89.41 & 68.42 & $-$20.99 & 61.98 & 62.16 & 64.50 & $+$2.34\\
% 0.50 & 0.99 & 89.62 & 73.41 & $-$16.21 & 67.64 & 67.86 & 70.25 & $+$2.39 \\ 
% 0.66 & 0.99 & 89.82 & 77.98 & $-$11.84 & 73.48 & 73.60 & 75.43 & $+$1.83 \\
% 0.75 & 0.99 & 89.70 & 79.41 & $-$10.29 & 76.46 & 76.53 & 77.70 & $+$1.17\\
% \bottomrule
% \end{tabular}
% \label{tab.gauss}
% \end{center}
% \end{table}

\begin{table}[!h]
\begin{center}
\caption{Evaluation on synthetic Gaussian data. `FS Acc.' denotes the accuracy of our feature separation method for $\mathbf{X}_2$. By removing non modality-general feature channels identified by Algorithm \ref{alg.sep}, we obtain a modality-general teacher with downgraded performance and its student with increasing accuracy; this validates our modality focusing hypothesis.}
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{$\gamma$} & \multirow{2}{*}{\makecell[c]{FS\\Acc.}} &
\multicolumn{2}{c}{Teacher Accuracy (\%)} & \multicolumn{3}{c}{Student Accuracy (\%)}\\
\cmidrule(lr){3-4}
\cmidrule(lr){5-7}
 & & Regular & Modality-general & No-KD & Regular & Modality-general \\
\midrule
% 0.25 & 0.90 & 89.70 & 64.84 & \dd24.86 & 59.29 & 59.46 & 61.01 & \uu 1.55\\
0.33 & 0.98 & 89.41 & 68.42 (\dd) & 61.98 & 62.16 & 64.50 (\uu)\\
0.50 & 0.99 & 89.62 & 73.41 (\dd) & 67.64 & 67.86 & 70.25 (\uu)\\ 
0.66 & 0.99 & 89.82 & 77.98 (\dd) & 73.48 & 73.60 & 75.43 (\uu) \\
0.75 & 0.99 & 89.70 & 79.41 (\dd) & 76.46 & 76.53 & 77.70 (\uu)\\
\bottomrule
\end{tabular}
\label{tab.gauss}
\end{center}
\end{table}

As shown in Table \ref{tab.gauss}, our proposed feature separation method can correctly identify modality-general features in input data (accuracy close to 1.0). Moreover, by removing non modality-general decisive feature channels, we can train a teacher that is specialized for distillation and obtain an improved student network. Since the modified teacher only relies on modality-general decisive features for prediction, we observe a accuracy loss in the teacher. However, the student network does not get affected and demonstrates increased accuracy for all choices of $\gamma$ instead. These results validate our proposed modality focusing hypothesis and shed light on how to utilize the hypothesis to facilitate the student network's learning process. 

\subsection{RAVDESS}\label{sec.expravdess}
RAVDESS~\citep{ravdess} is an audio-visual dataset containing 1,440 emotional utterances with 8 different emotion classes. We consider images as modality $1$ and audio as modality $2$. Teacher and student network are 3-layer CNNs. More details are provided in the Appendix. Since permutation is time-consuming at the model input level, we take middle-layer features (\ie, 128-dimensional features after the first linear layer) as input to Algorithm \ref{alg.sep}.
% \begin{wraptable}{l}{0.4\textwidth}
% \begin{center}
% \caption{Test Accuracy (\%) on RAVDESS Emotion Recognition. Teacher modality is audio and student modality is images. With identical model architecture, a modality-general teacher improves regular KD while a modality-specific teacher leads to a significantly worse student.}
% \begin{small}
% \begin{tabular}{c|ll}
% \toprule
% & & Acc. (\%) \\
% \midrule
%  Teacher & & 77.60\\
%  \midrule
% \multirow{4}{*}{Student}  & Regular & 77.22 \\
% & Modality-specific & 42.66 (\dd)\\
% & Random & 64.75\\
% & Modality-general & 78.28 (\uu)\\
% \bottomrule
% \end{tabular}
% \label{tab.ravdess}
% \end{small}
% \end{center}
% \end{wraptable}
After we obtain the saliency vector $\mathbf{p}\in\mathbb{R}^{128}$, we evaluate KD under four settings: (1) regular KD; (2) random: we randomly nullify 50\% of audio feature dimension, \ie, set the corresponding feature dimension to be its batch mean, which is identical for all samples in this batch. The student is trained to match predictions given by the ``randomly masked'' teacher; (3) modality-specific: we sort $\mathbf{p}$ in descending order, nullify the first 50\% feature dimension in the teacher and train a student subsequently; (4) modality-general: we sort $\mathbf{p}$ in ascending order, nullify the first 50\% feature dimension and perform KD. In this way, we remove modality-general decisive features in teacher's decision process in the third setting and remove non modality-general decisive features in the last setting. While we can not know the true value of $\gamma$ for each teacher, we know that $\gamma$ increases in the order of modality-specific, random and modality-general teacher. This allows us to justify the proposed modality focusing hypothesis. Results are averaged over 5 runs.

% We consider RGB images as modality $1$ and adopt a 3-layer CNN as the student network. Mel-scale Frequency Cepstral Coefficients (MFCCs) of audio are regarded as modality $2$ features, and we train a 3-layer CNN to be the audio teacher.

\begin{table}[!h]
\begin{center}
\caption{Test Accuracy (\%) on RAVDESS Emotion Recognition. Teacher modality is audio and student modality is images. With identical model architecture, a modality-general teacher improves regular KD while a modality-specific teacher leads to a significantly worse student.}
\begin{tabular}{c|cccc}
\toprule
\multirow{2}{*}{\makecell[c]{Teacher}} & \multicolumn{4}{c}{Student} \\
 & Regular & Modality-specific & Random & Modality-general \\
\midrule
77.60 & 77.22 & 42.66 (\dd) & 64.75 & 78.28 (\uu)\\
\bottomrule
\end{tabular}
\label{tab.ravdess}
\end{center}
\end{table}

As demonstrated in Table \ref{tab.ravdess}, a modality-specific teacher leads to a significantly downgraded student (\ie, accuracy drops from 77.22\% to 42.66\%). On the other hand, we observe an improved student (\ie, test accuracy increases to 78.28\%) after nullifying non general decisive features in the teacher (modality-general setting). This indicates the critical role of modality-general decisive features in distillation. A modality-general audio teacher can better transfer knowledge to the visual student as it discards audio-specific information not understandable by the student. 

\subsection{Event Classification on VGGSound}\label{sec.expvgg}
% VGGSound~\citep{chen2020vggsound} is a large-scale audio-video event classification dataset including over 200,000 video and 310 classes. We randomly choose 100 class including 56,614 audio-video pairs for training and 4,501 audio-video pairs for testing. We set modality 1 (\ie, student modality) as video and modality 2 (\ie, teacher modality) as audio. The student model is based on ResNet-18 with videos as input. To match 3D inputs, we simply replace all 2D convolution operations by 3D convolution operations of the ResNet-18~\citep{}. The teacher model is ResNet-18 with spectragram as input which we apply a short time Fourier transform on audio to generate. According to Algorithm \ref{alg.sep}, we need to permute the features of $\mathbb{X}_2$, if we simply regard the input audio or video as $X$, it faces slow permutation and distance calculation speed and a pixel may not be suitable to be regarded as decisive features or not. Therefore, we take the features from preliminary layers to permute. Then we got the saliency vector $\mathbf{p} \in \mathcal{R}^{512}$. We evaluate the utility of modality-general decisive feature in knowledge distillation under 5 settings: 1) naive KD 2) KD with feature aligned teacher 3) randomly nullify features in $\mathbf{p}$ 4) nullify the modality-general deceive features in $\mathbf{p}$ 5) nullify the non modality-general deceive features in $\mathbf{p}$. Although take the same model and input data, teachers in settings 3, 4, 5 generate different knowledge.

VGGSound~\citep{chen2020vggsound} is a large-scale audio-visual event classification dataset including over 200,000 video and 310 classes. We set modality 1 (\ie, student modality) as video and modality 2 (\ie, teacher modality) as audio. More experimental details are provided in the Appendix.  We take features before the last fully connected layer as input to Algorithm \ref{alg.sep} and obtain a 512-dimensional saliency vector $\mathbf{p}$. Similar to the previous experiment, we obtain a random, modality-specific and modality-general teacher by nullifying 75\% audio feature dimension according to $\mathbf{p}$. We experiment with two backbone architectures, ResNet-18 and ResNet-50~\citep{he2016deep}, and report results in Table \ref{tab:vggsound}.

% \begin{table}[!th]
% \begin{center}
% \caption{Test Accuracy (\%) on VGGSound Event Classification. GD Feat. denotes modality-general decisive features. Teacher modality is audio and student modality is video. We randomly remove or remove GD and Non-GD features to observe the effectiveness in KD.}
% \begin{tabular}{c|cccccc}
% \toprule
% \multirow{2}{*}{\makecell[c]{Teacher}} & \multicolumn{6}{c}{Student} \\
%  &Baseline & KD  &KD (Align) & Random   & \makecell[c]{GD Feat.} & \makecell[c]{Non GD Feat.} \\
% \midrule
% 29.86 & 29.86 & 30.62 & 30.95 (\uu) &30.99
%  & 24.98(\dd)& 31.88
% (\uu)\\
% \bottomrule
% \end{tabular}
% \label{tab:vggsound}
% \end{center}
% \end{table}

% \begin{table}[!th]
% \begin{center}
% \caption{Mean Average Precision (\%) on VGGSound Event Classification. Teacher modality is audio and student modality is video. The student learning from a modality-general teacher demonstrates best performance.}
% \begin{tabular}{c|cccc}
% \toprule
% \multirow{2}{*}{\makecell[c]{Teacher}} & \multicolumn{4}{c}{Student} \\
%  & Regular & Modality-specific & Random & Modality-general \\
% \midrule
% 29.86 & 30.62  & 24.98 (\dd) &30.99
% & 31.88
% (\uu)\\
% \bottomrule
% \end{tabular}
% \label{tab:vggsound}
% \end{center}
% \end{table}
As shown in the Table \ref{tab:vggsound},  modality-general decisive features play a critical role in multimodal KD. The student learning from a modality-specific teacher suffers from a major performance degradation. On the contrary, nullifying non \gd \ in the teacher improves the student performance from 30.62\% to 31.88\% (for ResNet-18) and from 38.78\% to 39.81\% (for ResNet-50).

Moreover, we provide an ablation study on the ratio of feature dimension that gets nullified in Fig. \ref{fig.abl_vgg}. We can see that there exists a sweet spot for modality-general KD. As the ratio increases, the student performance improves in the beginning. The improvement indicates that non \gd \ in the teacher are gradually discarded, which in turn results in a better student. Later, after all non general decisive information are removed, the nullifying process starts to hinder student performance as \gd \ get nullified as well. These results align well with our understanding of the modality Venn diagram and demonstrate the efficacy of our proposed Algorithm \ref{alg.sep}.

\begin{minipage}[!t]{\textwidth}
  \begin{minipage}[c]{0.6\textwidth}
    \centering
    \captionof{table}{Student mean Average Precision (\%) on VGGSound Event Classification. Teacher modality is audio and student modality is video. The student learning from a modality-general teacher demonstrates best performance. }
    % \begin{small}
    \begin{tabular}{lll}
\toprule
Model Architecture & ResNet-18  & ResNet-50 \\
\midrule
Teacher & 29.86 & 37.51\\
\cmidrule(lr){1-1}
 Regular & 30.62 & 38.78 \\
 Modality-specific & 24.98 (\dd) & 28.65 (\dd)\\
Random & 28.99 & 35.95\\
Modality-general & 31.88 (\uu) & 39.81(\uu)  \\
\bottomrule
\end{tabular}
% \end{small}
\label{tab:vggsound}
    \end{minipage}
    \hfill
    \begin{minipage}[c]{0.4\textwidth}
    \centering
    \includegraphics[width=0.8\linewidth]{figs/abl_v2.pdf}
    \captionof{figure}{Ablation study on nullified feature dimension ratio.}
    \label{fig.abl_vgg}
  \end{minipage}
  \end{minipage}
  
\noindent\textbf{Visualization of Modality-General Features.} As shown in Figure \ref{fig:cam}, we plot the class activation map (CAM) from all features and modality-general features. We find that if the model takes all video features for classification, the most interesting part of the images are the objects like the Saxophone or the baby. In contrast, if the model only takes modality-general features for classification, the most interesting part of the images are the the area of vocalization like the mouth of people.
\begin{figure}
    \centering
    \begin{tabular}{ccc}
         \includegraphics[width=0.2\textwidth]{./figs/visualization/17.png}\hspace{10mm}& \includegraphics[width=0.2\textwidth]{./figs/visualization/img1.png}& \includegraphics[width=0.2\textwidth]{./figs/visualization/img1_general.png} \\
         \includegraphics[width=0.2\textwidth]{./figs/visualization/24.png}\hspace{10mm}& \includegraphics[width=0.2\textwidth]{./figs/visualization/img2.png}& \includegraphics[width=0.2\textwidth]{./figs/visualization/img2_general.png} \\
         Image & All Features& Modality-General Features  
    \end{tabular}
    \caption{The class activation maps from all features (left) and the modality-general features (right). The class activation map from the modality-general features locate at the area of vocalization.}
    \label{fig:cam}
\end{figure}

% Modality-general KD steadily improves in the beginning and then decreases. This process aligns well with our understanding of the modality Venn diagram.

% We report the result on Table \ref{tab:vggsound}. We find that the alignment in teacher model between audio and video (eq \ref{eq.train}) slightly improve the accuracy of student model from 30.62 to 30.95. Randomly remove features keep similar performance of student after distillation. The performance significantly dropped if we remove general decisive feature. the In contrast, removing the non general decisive feature improve the performance from 30.95 to 31.88.

% \subsubsection{Ablation Study}


\subsection{Semantic Segmentation on NYU Depth V2}\label{sec.expnyu}
Finally, we revisit the example of NYU Depth V2 \citep{nyu} in Sec. \ref{sec.failurecase}. Here the two modalities (\ie, RGB and depth images) have large similarity and can be taken as input for a single model. Therefore, we design a modality-agnostic teacher model for distillation. This can be seen as an alternative way to demonstrate the modality focusing hypothesis apart from our proposed feature separation method.

We adopt a teacher network that takes depth images as input to transfer knowledge to an RGB student. As shown in Table \ref{tab.nyu}, regular KD (\ie, using the modality-specific teacher) does not bring many advantages: the student achieves a similar mIoU compared with a RGB model without KD. Based on this result, one might easily blame the failure of KD on teacher accuracy and assume that KD is not effective because the depth teacher itself yields poor performance (\ie, has an mIoU of 37.33\%).
% \vspace{-5mm}
% We design a modality-general teacher that is trained on both RGB and depth images to emphasize modality-general decisive features in its decision process.
\begin{table}[!t]
\begin{center}
\caption{Mean Intersection over Union (mIoU) on NYU Depth RGB-D Semantic Segmentation. Teacher modality is depth images and student modality is RGB images. Compared with regular crossmodal KD (\ie, using a modality-specfic depth teacher), a modality-general teacher is more suitable for distillation and leads to a better student.}
% \vspace{1mm}
\begin{tabular}{ccccc}
\toprule
 & \multicolumn{2}{c}{Teacher} & \multicolumn{2}{c}{Student} \\
 & Modality & mIoU (\%) & Modality & mIoU (\%) \\
 \midrule
 No-KD & - & - & \texttt{RGB} & 46.36\\
 Modality-specific-KD & \texttt{D} & 37.33 & \texttt{RGB} & 46.89 \\
 Modality-general-KD & \texttt{RGB/D} & 37.47 & \texttt{RGB} & 47.93\\
\bottomrule
\end{tabular}
\label{tab.nyu}
\end{center}
\end{table}

The modality focusing hypothesis motivates us to think otherwise. We train a modality-general teacher that receives both RGB and depth images as input. Similar to ~\citep{girdhar2022omnivore}, we use one single model to predict labels for two modalities with exactly same parameters. Note that the model architecture is identical to the previous modality-specific teacher to ensure a fair comparison. In this way, the teacher is forced to extract modality-general decisive features for prediction rather than rely on depth-specific features as it also takes RGB images as input. While we do not observe difference in teacher performance, the new teacher is categorized for distillation and leads to a better depth student (\ie, student mIoU increases from 46.36\% to 47.93\%). These results show how our modality focusing hypothesis can indeed help diagnose failure of crossmodal KD and improve it. 

% These results detach the efficacy of KD from teacher performance and lend support to the modality focusing hypothesis.

% We transform depth images to HHA images first and treat these two kinds of images identically. In other words, a training batch may contain both RGB and depth images.
% Justify Modality Focusing Hypothesis: Synthetic Gaussian Dataset

% Or alternatively, the 'Justify xxxxx' could be put in the first sentence of every subsection.

% \begin{itemize}
%     \item demonstrate 4.2
%     \item use synthetic data to show that our proposed approach can correctly identify alpha and beta. 
% \end{itemize}

% Justify Implication 1: RAVDESS + VGG-Sound
% \begin{itemize}
%     \item demonstrate 4.3.(1)
%     \item modify data to verify our hypothesis
% \end{itemize}
% Justify Implication 2: NYU Depth V2 + MM IMDB 
% \begin{itemize}
%     \item demonstrate 4.3.(2) 
%     \item based on the hypothesis, improve teacher model
%     \item train two versions of teacher model, one normal, the other focusing on common features, compare student performance
% \end{itemize}
